Shuffling Gradient-Based Methods for Nonconvex-Concave Minimax Optimization

This paper aims at developing novel shuffling gradient-based methods for tackling two classes of minimax problems: nonconvex-linear and nonconvex-strongly concave settings. The first algorithm addresses the nonconvex-linear minimax model and achieves the state-of-the-art oracle complexity typically observed in nonconvex optimization. It also employs a new shuffling estimator for the "hyper-gradient", departing from standard shuffling techniques in optimization. The second method consists of two variants: semi-shuffling and full-shuffling schemes. These variants tackle the nonconvex-strongly concave minimax setting. We establish their oracle complexity bounds under standard assumptions, which, to our best knowledge, are the best-known for this specific setting. Numerical examples demonstrate the performance of our algorithms and compare them with two other methods. Our results show that the new methods achieve comparable performance with SGD, supporting the potential of incorporating shuffling strategies into minimax algorithms.

==> sections/SGM_main_paper_refs.tex <==
\begin{thebibliography}{10}

\bibitem{arjovsky2017wasserstein}
M.~Arjovsky, S.~Chintala, and L.~Bottou.
\newblock Wasserstein generative adversarial networks.
\newblock In {\em International Conference on Machine Learning}, pages
  214--223, 2017.

\bibitem{azar2017minimax}
M.~G. Azar, I.~Osband, and R.~Munos.
\newblock Minimax regret bounds for reinforcement learning.
\newblock In {\em International Conference on Machine Learning}, pages
  263--272. PMLR, 2017.

\bibitem{Ben-Tal2009}
A.~Ben-Tal, L.~El~Ghaoui, and A.~Nemirovski.
\newblock {\em {R}obust optimization}.
\newblock Princeton University Press, 2009.

\bibitem{beznosikov2023stochastic}
A.~Beznosikov, E.~Gorbunov, H.~Berard, and N.~Loizou.
\newblock Stochastic gradient descent-ascent: Unified theory and new efficient
  methods.
\newblock In {\em International Conference on Artificial Intelligence and
  Statistics}, pages 172--235. PMLR, 2023.

\bibitem{bhatia2020online}
K.~Bhatia and K.~Sridharan.
\newblock Online learning with dynamics: {A} minimax perspective.
\newblock {\em Advances in Neural Information Processing Systems},
  33:15020--15030, 2020.

\bibitem{CC01a}
C.-C. Chang and C.-J. Lin.
\newblock {LIBSVM}: {A} library for {S}upport {V}ector {M}achines.
\newblock {\em ACM Transactions on Intelligent Systems and Technology},
  2:27:1--27:27, 2011.

\bibitem{cho2022sgda}
H.~Cho and C.~Yun.
\newblock {SGDA} with shuffling: faster convergence for nonconvex-P{\L} minimax optimization.
\newblock {\em The 11th International Conference on Learning Representations}, pp. 1--10, 2022.

\bibitem{das2022sampling}
A.~Das, B.~Sch{\"o}lkopf, and M.~Muehlebach.
\newblock Sampling without replacement leads to faster rates in finite-sum
  minimax optimization.
\newblock {\em Advances in Neural Information Processing Systems},
  35:6749--6762, 2022.

\bibitem{dempe2002foundations}
S.~Dempe.
\newblock {\em Foundations of Bilevel Programming}.
\newblock Springer Science \& Business Media, 2002.

\bibitem{driggs2019bias}
D.~Driggs, J.~Liang, and C.-B. Sch{\"o}nlieb.
\newblock On biased stochastic gradient estimation.
\newblock {\em Journal of Machine Learning Research}, vol. 23, no. 24, pp. 1--43, 2022.

\bibitem{emmanouilidis2024stochastic}
K.~Emmanouilidis, R.~Vidal, and N.~Loizou.
\newblock Stochastic extragradient with random reshuffling: Improved
  convergence for variational inequalities.
\newblock In {\em International Conference on Artificial Intelligence and
  Statistics}, pages 3682--3690. PMLR, 2024.

\bibitem{gidel2018variational}
G.~Gidel, H.~Berard, G.~Vignoud, P.~Vincent, and S.~Lacoste-Julien.
\newblock A variational inequality perspective on generative adversarial
  networks.
\newblock {\em International Conference on Learning Representations}, pp. 1--10, 2019.

\bibitem{goodfellow2014generative}
I.~Goodfellow, J.~Pouget-Abadie, M.~Mirza, B.~Xu, D.~Warde-Farley, S.~Ozair,
  A.~Courville, and Y.~Bengio.
\newblock Generative adversarial nets.
\newblock In {\em Advances in neural information processing systems}, pages
  2672--2680, 2014.

\bibitem{gorbunov2022stochastic}
E.~Gorbunov, H.~Berard, G.~Gidel, and N.~Loizou.
\newblock Stochastic extragradient: General analysis and improved rates.
\newblock In {\em International Conference on Artificial Intelligence and
  Statistics}, pages 7865--7901. PMLR, 2022.

\bibitem{hamedani2018iteration}
E.~Y. Hamedani, A.~Jalilzadeh, N.~S. Aybat, and U.~V. Shanbhag.
\newblock Iteration complexity of randomized primal-dual methods for
  convex-concave saddle point problems.
\newblock {\em arXiv preprint arXiv:1806.04118}, 2018.

\bibitem{haochen2018random}
J.~Z. HaoChen and S. Sra.
\newblock Random shuffling beats SGD after finite epochs.
\newblock {\em International Conference on Machine Learning}, pp.  2624--2633, 2019.

\bibitem{ho2022game}
E.~Ho, A.~Rajagopalan, A.~Skvortsov, S.~Arulampalam, and M.~Piraveenan.
\newblock Game theory in defence applications: {A} review.
\newblock {\em Sensors}, 22(3):1032, 2022.

\bibitem{hsieh2020explore}
Y.~Hsieh, F.~Iutzeler, J.~Malick, and P.~Mertikopoulos.
\newblock Explore aggressively, update conservatively: Stochastic extragradient
  methods with variable stepsize scaling.
\newblock {\em Advances in Neural Information Processing Systems},
  33:16223--16234, 2020.

\bibitem{jabbar2021survey}
Abdul Jabbar, Xi~Li, and Bourahla Omar.
\newblock A survey on generative adversarial networks: Variants, applications,
  and training.
\newblock {\em ACM Computing Surveys (CSUR)}, 54(8):1--49, 2021.

\bibitem{lan2020first}
G.~Lan.
\newblock {\em First-order and Stochastic Optimization Methods for Machine
  Learning}.
\newblock Springer, 2020.

\bibitem{lin2022distributionally}
F.~Lin, X.~Fang, and Z.~Gao.
\newblock Distributionally robust optimization: {A} review on theory and
  applications.
\newblock {\em Numerical Algebra, Control \& Optimization}, 12(1):159, 2022.

\bibitem{loizou2021stochastic}
N.~Loizou, H.~Berard, G.~Gidel, I.~Mitliagkas, and S.~Lacoste-Julien.
\newblock Stochastic gradient descent-ascent and consensus optimization for
  smooth games: {C}onvergence analysis under expected co-coercivity.
\newblock {\em Advances in Neural Information Processing Systems},
  34:19095--19108, 2021.

\bibitem{luo2020stochastic}
L.~Luo, H.~Ye, and T.~Zhang.
\newblock Stochastic recursive gradient descent ascent for stochastic
  nonconvex-strongly-concave minimax problems.
\newblock {\em Advances in Neural Information Processing Systems}, vol. 33, pp. 20566--20577, 2020.

\bibitem{Luo1996}
Z.~Luo, J.~Pang, and D.~Ralph.
\newblock {\em {M}athematical {P}rograms with {E}quilibrium {C}onstraints}.
\newblock Cambridge {U}niversity {P}ress, Cambridge, 1996.

\bibitem{madry2018towards}
A.~Madry, A.~Makelov, L.~Schmidt, D.~Tsipras, and A.~Vladu.
\newblock Towards deep learning models resistant to adversarial attacks.
\newblock In {\em International Conference on Learning Representations}, 2018.

\bibitem{meng2019convergence}
Q.~Meng, W.~Chen, Y.~Wang, Z.-M. Ma, and T.-Y. Liu.
\newblock Convergence analysis of distributed stochastic gradient descent with
  shuffling.
\newblock {\em Neurocomputing}, 337:46--57, 2019.

\bibitem{mishchenko2020random}
K.~Mishchenko, A.~Khaled, and P.~Richt{\'a}rik.
\newblock Random reshuffling: Simple analysis with vast improvements.
\newblock {\em Advances in Neural Information Processing Systems},
  33:17309--17320, 2020.

\bibitem{mishchenko2022proximal}
K.~Mishchenko, A.~Khaled, and P.~Richt{\'a}rik.
\newblock Proximal and federated random reshuffling.
\newblock In {\em International Conference on Machine Learning}, pages
  15718--15749. PMLR, 2022.

\bibitem{Nesterov2004}
Y.~Nesterov.
\newblock {\em {I}ntroductory lectures on convex optimization: {A} basic
  course}, volume~87 of {\em Applied Optimization}.
\newblock Kluwer Academic Publishers, 2004.

\bibitem{nguyen2020unified}
L.~M. Nguyen, Q.~Tran-Dinh, D.~T. Phan, P.~H. Nguyen, and M.~van Dijk.
\newblock A unified convergence analysis for shuffling-type gradient methods.
\newblock {\em Journal of Machine Learning Research}, 22(207):1--44, 2021.

\bibitem{palaniappan2016stochastic}
B.~Palaniappan and F.~Bach.
\newblock Stochastic variance reduction methods for saddle-point problems.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  1416--1424, 2016.

\bibitem{Safran2019HowGoodSGDShuffling}
I.~Safran and O.~Shamir.
\newblock How good is {SGD} with random shuffling?
\newblock {\em Conference on Learning Theory}, pp. 3250--3284, 2020.

\bibitem{shapiro2002minimax}
A.~Shapiro and A.~Kleywegt.
\newblock Minimax analysis of stochastic problems.
\newblock {\em Optim. Methods Softw.}, 17(3):523--542, 2002.

\bibitem{TranDinh2020f}
Q.~Tran-Dinh, D.~Liu, and L.~M. Nguyen.
\newblock Hybrid variance-reduced {SGD} algorithms for nonconvex-concave
  minimax problems.
\newblock {\em The 34th Conference on Neural Information Processing Systems
  (NeurIPs 2020)}, 2020.

\bibitem{wang2021adversarial}
J.~Wang, T.~Zhang, S.~Liu, P.-Y. Chen, J.~Xu, M.~Fardad, and B.~Li.
\newblock Adversarial attack generation empowered by min-max optimization.
\newblock {\em Advances in Neural Information Processing Systems},
  34:16020--16033, 2021.

\bibitem{wang2017stochastic}
M.~Wang, E.~Fang, and L.~Liu.
\newblock Stochastic compositional gradient descent: algorithms for minimizing
  compositions of expected-value functions.
\newblock {\em Math. Program.}, 161(1-2):419--449, 2017.

\bibitem{yang2020global}
J.~Yang, N.~Kiyavash, and N.~He.
\newblock Global convergence and variance-reduced optimization for a class of
  nonconvex-nonconcave minimax problems.
\newblock {\em arXiv preprint arXiv:2002.09621}, 2020.

\bibitem{ying2017convergence}
B.~Ying, K.~Yuan, and A.~H. Sayed.
\newblock Convergence of variance-reduced stochastic learning under random
  reshuffling.
\newblock {\em arXiv preprint arXiv:1708.01383}, 2(3):6, 2017.

\bibitem{zhang2020stochastic}
J.~Zhang and L.~Xiao.
\newblock Stochastic variance-reduced prox-linear algorithms for nonconvex
  composite optimization.
\newblock {\em Mathematical Programming}, pp. 1--43, 2022.

\bibitem{zhang2021multi}
K.~Zhang, Z.~Yang, and T.~Ba{\c{s}}ar.
\newblock Multi-agent reinforcement learning: {A} selective overview of
  theories and algorithms.
\newblock {\em Handbook of reinforcement learning and control}, pages 321--384,
  2021.

\bibitem{zhao2010convex}
L.~Zhao, M.~Mammadov, and J.~Yearwood.
\newblock From convex to nonconvex: a loss function analysis for binary
  classification.
\newblock In {\em IEEE International Conference on Data Mining Workshops
  (ICDMW)}, pages 1281--1288. IEEE, 2010.

\bibitem{zhao2019optimal}
R.~Zhao.
\newblock Optimal stochastic algorithms for convex-concave saddle-point
  problems.
\newblock {\em arXiv preprint arXiv:1903.01687}, 2019.

\end{thebibliography}

